YA-TA: Towards Personalized Question-Answering Teaching Assistants using Instructor-Student Dual Retrieval-augmented Knowledge Fusion

Engagement between instructors and students plays a crucial role in enhancing students'academic performance. However, instructors often struggle to provide timely and personalized support in large classes. To address this challenge, we propose a novel Virtual Teaching Assistant (VTA) named YA-TA, designed to offer responses to students that are grounded in lectures and are easy to understand. To facilitate YA-TA, we introduce the Dual Retrieval-augmented Knowledge Fusion (DRAKE) framework, which incorporates dual retrieval of instructor and student knowledge and knowledge fusion for tailored response generation. Experiments conducted in real-world classroom settings demonstrate that the DRAKE framework excels in aligning responses with knowledge retrieved from both instructor and student sides. Furthermore, we offer additional extensions of YA-TA, such as a Q&A board and self-practice tools to enhance the overall learning experience. Our video is publicly available.

==> figures/geval/comprehensiveness.tex <==
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.98\linewidth]{images/geval/comprehensiveness.png}
    \caption{G-Eval prompt used to assess comprehensiveness}
    \label{fig:comprehensiveness}
\end{figure}

==> figures/geval/groundedness.tex <==
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.98\linewidth]{images/geval/groundedness.png}
    \caption{G-Eval prompt used to assess groundedness}
    \label{fig:groundedness}
\end{figure}

==> figures/geval/helpfulness.tex <==
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.98\linewidth]{images/geval/helpfulness.png}
    \caption{G-Eval prompt used to assess helpfulness}
    \label{fig:helpfulness}
\end{figure}

==> figures/geval/overall.tex <==
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.98\linewidth]{images/geval/overall.png}
    \caption{G-Eval prompt used to assess overall personalization ability}
    \label{fig:overall}
\end{figure}

==> figures/prompts/grading.tex <==
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.98\linewidth]{images/prompts/grading.png}
    \caption{Prompt used to grade the response of the student}
    \label{fig:grading}
\end{figure*}

==> figures/prompts/plan.tex <==
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.98\linewidth]{images/prompts/plan.png}
    \caption{Prompt used in the planning process before generating final response}
    \label{fig:plan}
\end{figure*}

==> figures/prompts/quiz.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.98\linewidth]{images/prompts/quiz-generation.png}
    \caption{Prompt used to generate quiz}
    \label{fig:quiz}
\end{figure*}

==> figures/prompts/response.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.98\linewidth]{images/prompts/response-generation.png}
    \caption{Prompt used to generate the response}
    \label{fig:response}
\end{figure*}

==> figures/prompts/retriever.tex <==
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.98\linewidth]{images/prompts/retriever.png}
    \caption{Prompt used to retrieve relevant segments from the lecture of instructor}
    \label{fig:retriever}
\end{figure*}


==> tables/case_study_korean.tex <==
\begin{table}[ht]
    \small
    \begin{tabular}{p{\linewidth}}
    \toprule
        \textsc{\textbf{Social Science}} \\
    \midrule
        \info \space \textbf{Student Information} \\
        Major: Artificial Intelligence \\ Degree: Graduate Student \\ Semester: 3 \\ 
        Grade: (Data Structures, A), (Algorithms, A+), ... \\ 
    \midrule
        \query \space \textbf{Student's Query} \\
        자본주의와 민주주의의 관계에 대해서 설명해줘. \\
    \midrule
        \query \space \textbf{Translated Student's Query} \\
        Explain the relationship between capitalism and democracy. \\
    \midrule
        \evidence \space \textbf{Evidence} \\
        그러나 \textbf{자본주의가 없는 상황에서 민주주의를 유지하는 것은 어렵다}고 일반적으로 보고 있습니다. (895.82, 904.66) timestamp:(start:819.96, end:904.66) ... \\
    \midrule
        \evidence \space \textbf{Translated Evidence} \\
        However, \textbf{it is generally considered difficult to maintain democracy in the absence of capitalism}. timestamp: (start: 819.96, end: 904.66) ... \\
    \midrule
        \YATAresponse \space \textbf{YA-TA response} \\
        자본주의와 민주주의는 서로 상호작용하는 관계에 있습니다... \\
        \textbf{민주주의가 지속적으로 유지되고 발전하는 데에 자본주의가 중요한 역할}을 합니다... \\
        인공지능 분야에서도 이러한 관계는 명확하게 나타납니다. 예를 들어, 자본주의 시장에서는 \textbf{AI 기술의 발전이 경쟁을 통해 촉진되며, 이는 혁신과 경제 성장을 가져옵니다}. \\
    \midrule
        \YATAresponse \space \textbf{Translated YA-TA response} \\
        Capitalism and democracy interact with each other... \\
        \textbf{capitalism plays an important role in the continuous maintenance and development of democracy.}... \\
        In the field of artificial intelligence, this relationship is particularly evident. For example, in a capitalist market, \textbf{the advancement of AI technology is driven by competition, leading to innovation and economic growth}. \\
    \midrule
        \GPTresponse \space \textbf{GPT-4o response} \\
        자본주의와 민주주의는 현대 사회에서 중요한 두 가지 개념으로, 각각 경제와 정치 체제를 나타냅니다... \\
        자본주의와 민주주의는 서로 다른 영역에서 작동하지만, 현대 사회에서 종종 함께 나타납니다. \\
    \midrule
        \GPTresponse \space \textbf{Translated GPT-4o response} \\
        Capitalism and democracy are two important concepts in modern society, representing economic and political systems, respectively ... \\
        The way capitalism and democracy are combined can vary widely depending on each country's historical and cultural context. \\
    \bottomrule
    \end{tabular}
    \label{tab:case_korean}
\caption{Response from YA-TA on a Korean Lecture}
\end{table}

==> tables/quiz_generation.tex <==
\begin{table*}
    \small
    \centering
    \begin{tabular}{p{14cm}}
    \toprule
    \textbf{Prompt} \\
    \midrule
    % Given a review written by you, summarize what you liked and disliked about the movie, under [Like] and [Dislike] respectively. If there is nothing to mention about like/dislike, simply write "None." under the corresponding tag.
    % \\
    % \\
    % Here is the movie review written by you: \\ \{review\} \\

    Assume you are a professor.....blah blah \\
    \\
    \#\# Lecture Script \\
    \{context\} \\
    \\
    \#\# Summary \\
    \{syllabus\} \\
    

    \bottomrule
    \end{tabular}
    \caption{The prompt for quiz generation.}
    \label{tab:quiz_generation}
\end{table*}
